Efficient Image Reconstruction Architecture for Neutral Atom Quantum Computing

In recent years, neutral atom quantum computers (NAQCs) have attracted a lot of attention, primarily due to their long coherence times and good scalability. One of their main drawbacks is their comparatively time-consuming control overhead, with one of the main contributing procedures being the detection of individual atoms and measurement of their states, each occurring at least once per compute cycle and requiring fluorescence imaging and subsequent image analysis. To reduce the required time budget, we propose a highly-parallel atom-detection accelerator for tweezer-based NAQCs. Building on an existing solution, our design combines algorithm-level optimization with a field-programmable gate array (FPGA) implementation to maximize parallelism and reduce the run time of the image analysis process. Our design can analyze a 256$\times$256-pixel image representing a 10$\times$10 atom array in just 115 $\mu$s on a Xilinx UltraScale+ FPGA. Compared to the original CPU baseline and our optimized CPU version, we achieve about 34.9$\times$ and 6.3$\times$ speedup of the reconstruction time, respectively. Moreover, this work also contributes to the ongoing efforts toward fully integrated FPGA-based control systems for NAQCs.

==> chapters/algorithm.tex <==
\section{Algorithm}\label{chapters:algorithm}
The spatial distribution of photons that are gathered by the camera can be represented as the convolution of the brightness at each atom location with the \ac{PSF}, which represents the response of the optical imaging system to a point-like light source or unit impulse~\cite{gualdron2024learning}. Since the resulting values are discretized into pixel values and as there are, assuming a negligible background illumination, only a certain number of point-like light sources, this convolution can be simplified as the sum of each atom site's \ac{PSF} multiplied by its brightness~\cite{Wei:1}.

\citeauthor{Winklmann:1} denote the expected number of photoelectrons registered at pixel $x$ as
\begin{equation}
    \lambda(x,\gamma) = b + \sum_{i=0}^nPSF_i(x) \cdot\gamma_i
    \label{equation:pixelValue}
\end{equation}
for a background illumination $b$ and $n$ atom locations, each of which being described by its \ac{PSF} $PSF_i(x)$ and brightness $\gamma_i$~\cite{Winklmann:1}.

The chosen state-reconstruction algorithm is based on the assumption that, since this equation is linear, we can find an inverse \ac{PSF} that will reconstruct the initial brightnesses from the pixel values of our fluorescence image. To do so, the Moore-Penrose inverse of the \ac{PSF} is calculated and, for each atom site, multiplied element-wise with the image details of equal size, centered around the location in question. The sum of this multiplication serves as the emission value, which, using a threshold, can be used to determine whether each site contains an atom or not~\cite{Wei:1}.
\subsection{Calibration}
As \citeauthor{Wei:1} states, the acquisition of the \ac{PSF}'s inverse is the most time-consuming aspect of the calculation~\cite{Wei:1}. However, the \ac{PSF} hardly changes unless the setup itself changes. As such, it does not need to be updated every time we run the calculation. Instead, we relocate it, along with other tasks that don't require execution during every cycle, to a preceding calibration stage where execution time is less critical.

Being fed an exemplary set of images, the calibration procedure automatically detects the position and angle of the grid of atom location, the \ac{PSF} at each atom site, and calculates the inverse and detection threshold.
\subsection{Runtime}
At runtime, we only execute those parts of the calculation that change non-negligibly for each compute cycle. Since the only variable that this applies to is the fluorescence image itself, the only calculation that requires execution at runtime is the element-wise multiplication with the projection kernel and subsequent summation and thresholding. 

\subsection{Optimization}
% If we want to produce a solution that is useful to as large a user group as possible, it is important to offer usage on standard platforms. 
Since we want to produce a solution that is capable of being integrated into an \ac{FPGA}-based control system, it is not efficient to directly adopt the original algorithm~\cite{Wei:1}, which is inherently serial and algorithmically complicated. As such, we first follow the hardware–software co-design approach to reformulate and optimize the algorithm to make it execute efficiently on \acp{CPU} and, optionally, \acp{GPU}. Within our development, we observe that, since the sections of the program that are suited to run on \ac{GPU} are already comparatively fast and the transfer of data from \ac{CPU} to \ac{GPU} takes a non-negligible amount of time, an advantage of using this version could not consistently be established. As such, we will only use the \ac{CPU} version in the following chapters, referred to as the \ac{CPU}-baseline.

Due to the algorithm's focus on far smaller atom spacings, some aspects of it, such as the phase estimation, are superfluous or excessive for tweezer-based setups (the setup used in this work). Therefore, we refine it further to a tailor-fit solution for larger spacings running exclusively on \ac{CPU}. We also restructure the algorithm to expose inherent parallelism and simplify control flow. Instead of deploying parallel sections to a \ac{GPU}, we elect to employ OpenMP in order to utilize parallelization capabilities without suffering the drawback of transfer times between the two devices. We will refer to this version as the \ac{CPU}-optimized one, which is the foundation for the subsequent design of the \ac{FPGA} accelerator. It is to be noted that, while practically indistinguishable in their output for this use case, the \ac{CPU}-baseline and \ac{CPU}-optimized versions do not offer identical functionality, and any performance improvements do come at the cost of reduced adaptability to constraints such as smaller atom spacings and phase drift.

==> chapters/discussion.tex <==
\section{Discussion}
\label{chapter:diss}
As demonstrated in this work, \ac{FPGA}-based atom detection accelerators represent a significant milestone in the state preparation and readout of \acp{NAQC}, providing opportunities for low-latency image analysis and mid-circuit measurement. Nevertheless, we do not claim that every lab and every experiment that images atoms requires an \ac{FPGA}-based solution. We see that many setups require flexibility and the possibility to intervene at any point. Especially experiments on high-density lattice-based atom arrays, three-dimensional structure, and other cutting-edge ideas, at this point, typically require the flexibility that only a software-only solution can provide. Instead, we envision our hardware solution as part of the control system for well-explored conditions where human intervention is obsolete. As \ac{NAQC} is right at the edge of being capable of offering value in production environments, we deem fully integrated control hardware as a necessity for the continued success of this modality.

==> chapters/relatedWork.tex <==
\section{Related Work}
\label{chapters:rlw}
% The need for investigating preexisting work for our endeavor is twofold. Firstly, we have to investigate the type of algorithm best suited to our use case. It needs to be precise and generally suited for deployment on \ac{FPGA}. Secondly, the existence of comparable solutions on \acp{FPGA} will be investigated to see whether such an integrated approach has already been implemented elsewhere. 
\subsection{Atom Detection Algorithm}
Deconvolution algorithms have been extensively employed to solve atom detection tasks. 
% In searching for the deconvolution algorithm of choice for our project, we mostly relied on previous work that compared several potential algorithms in terms of their precision and time demands. 
\citeauthor{Rooij:1} compare several potential solutions, with Richardson-Lucy performing the best in terms of detection precision, closely followed by Wiener deconvolution. Expanding on their algorithm repertoire, \citeauthor{Winklmann:1} introduce several more complicated fit-for-purpose algorithms like a global non-linear least-squares solver and \citeauthor{Wei:1}'s state-reconstruction library. They come to the conclusion that there is a clear tradeoff between precision and algorithm execution time \cite{Winklmann:1}. 

Out of the presented possibilities, we deem \citeauthor{Wei:1}'s projection-based state-reconstruction algorithm as the most suitable, as it performs very close to the overall most precise global solver while requiring a hugely decreased execution time. Originally aimed at state detection in lattices to prepare a Bose-Einstein condensate \cite{Wei:1}, some of its features, such as phase detection and individual projection kernels based on sub-pixel position, seem to be excessive for setups with well-separated atom locations. With the omission of these procedures, its perceived disadvantage of being conceptually comparatively complex dissolves, leaving behind only a number of element-wise matrix multiplications, as we will explain in section~\ref{chapters:algorithm}. The fact that we deal with a fairly straightforward calculation that is repeated once per atom site paves the way for a pipelined execution on the \ac{FPGA}.

\subsection{Deconvolution on FPGAs}
To the best of our knowledge, only a limited number of prior works have explored \ac{FPGA}-based deconvolution methods for reducing computational latency. Several Richardson–Lucy accelerators~\cite{Karine_RL_FPGA,RL_FPGA1,RL_FPGA2} have been proposed for motion and hyperspectral image reconstruction. However, due to the algorithm’s computational intensity, these approaches face scalability challenges on \acp{FPGA}, particularly with large kernel sizes or high-resolution input images. In this paper, we build our accelerator based on the mentioned state-reconstruction algorithm~\cite{Wei:1}, which primarily relies on convolution operations. In this case, we can benefit from resource multiplexing and parallel computation, achieving improvements in both latency and hardware efficiency. 
